Distributed Maximum Matching Verification in CONGEST

We study the maximum cardinality matching problem in a standard distributed setting, where the nodes $V$ of a given $n$-node network graph $G=(V,E)$ communicate over the edges $E$ in synchronous rounds. More specifically, we consider the distributed CONGEST model, where in each round, each node of $G$ can send an $O(\log n)$-bit message to each of its neighbors. We show that for every graph $G$ and a matching $M$ of $G$, there is a randomized CONGEST algorithm to verify $M$ being a maximum matching of $G$ in time $O(|M|)$ and disprove it in time $O(D + \ell)$, where $D$ is the diameter of $G$ and $\ell$ is the length of a shortest augmenting path. We hope that our algorithm constitutes a significant step towards developing a CONGEST algorithm to compute a maximum matching in time $\tilde{O}(s^*)$, where $s^*$ is the size of a maximum matching.

==> algorithm.tex <==
\section{Proof of the Main Theorem}
\label{sec:algo}

We conclude by presenting the details of the main algorithm that
turns the linear-time algorithm of \Cref{lemma:pathalg} to find and
augment along a shortest augmenting path into an $O(s^*\log s^*)$-time
\CONGEST algorithm to compute a maximum matching (and thus prove
\Cref{thm:main}, our main theorem). We start with a simple
deterministic linear-time algorithm to compute a maximal matching.

\begin{lemma}\label{lemma:maximalmatching}
  Let $G=(V,E)$ be an undirected graph and let $s^*$ be the size of a
  maximum matching of $G$ ($s^*$ is now known to the nodes). There is
  a deterministic $O(s^*)$-round \CONGEST algorithm to compute a
  maximal matching $M$ of $G$. Further, at the end of the algorithm,
  all nodes know $|M|$.
\end{lemma}
\begin{proof}
  Let $D$ be the diameter of $G$. First note that
  $s^*\geq \lfloor D/2\rfloor$ as $G$ contains a shortest path $P$ of
  length $D$ and any matching of $P$ is also a matching of $G$. We can
  therefore afford to first use a standard $O(D)$-time algorithm to
  elect a leader $r\in V$ and to compute a breadth first search (BFS)
  tree $T$ of $G$, which is rooted at $r$ (for such an algorithm, see,
  e.g., \cite{peleg00}). Let $D_T=\Theta(D)$ be the depth of the
  spanning tree $T$. Note that the value of $D_T$ is known after
  computing $T$. Our maximal matching algorithm starts with
  $M=\emptyset$ and it consists of phases of $O(D_T)$ rounds where in
  each phase, at least $D_T$ edges are added to the matching $M$. In
  each phase, we first do $D_T$ steps of the following simple greedy
  algorithm. Assume that each edge has a unique ID (e.g., derived by
  combining the IDs of the two nodes of the edge). Let $F$ be the set
  of edges that connect two unmatched nodes (i.e., $F$ is the set of
  edges that can still be added to the matching). In each greedy step,
  we add each edge of $F$ with an ID that is larger than the IDs of
  all adjacent edges in $F$. Note that this guarantees that we never
  add adjacent edges and we thus always have a matching. As long as
  the matching is not maximal, each greedy step further adds at least
  one more edge to the matching (the largest ID edge in $F$). At the
  end of the phase, we use the BFS tree to compute the size of the
  current matching and to check whether the current matching is
  already maximal. The algorithm terminates if we detect that the
  matching is maximal. Each greedy step can clearly be implemented in
  $O(1)$ rounds in the \CONGEST model. A single phase can therefore be
  implemented in time $O(D_T)$. Further, each phase either ends with a
  maximal matching or it adds at least $D_T$ new edges to the
  matching. The total time complexity of the algorithm is therefore at
  most $\lceil s^*/D_T\rceil \cdot O(D_T)=O(s^*)$ (because we have
  $s^* = \Omega(D_T)$).
\end{proof}

We remark that in most cases, there are much more efficient algorithms
to compute a maximal matching. However, \Cref{lemma:maximalmatching}
is sufficiently fast for what we need and it also does the right thing
if the value of $s^*$ is very small. The following is a simple
corollary of \Cref{lemma:maximalmatching}

\begin{corollary}\label{cor:matchingsize}
  Let $G=(V,E)$ be an undirected graph and let $s^*$ be the size of a
  maximum matching. There is an $O(s^*)$-time deterministic algorithm
  to compute a value $S$ such that $s^*\leq S \leq 2s^*$.
\end{corollary}
\begin{proof}
  Follows directly from \Cref{lemma:maximalmatching} and the fact that
  a maximal matching is a $1/2$-approximation of a maximum matching.
\end{proof}

The following lemma is a classic result due to Hopcroft and Karp~\cite{hopkarp}.
\begin{lemma}[\hspace*{-3px} \cite{hopkarp}]\label{lem:aug-size}
  Let $G=(V,E)$ be a graph with maximum matching size $s^*$ and let
  $M$ be an arbitrary matching of $G$.
  If $|M|<s^*$, there exists an augmenting path of length less than
  $2s^*/(s^*-|M|)$ w.r.t.\ $M$ in $G$.		 
\end{lemma}	

\begin{algorithm}[t]
  \caption{\texttt{Maximum Matching $(G,S)$}}\label{alg:maximum-matching}
  \SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
  \Input{Graph $G$ and an upper bound $S$ on the size of its maximum matching}
  \Output{A maximum matching of $G$}
  \BlankLine
  $M \leftarrow \emptyset$;\\
  \For{$j=1$ to $\ceil{\log S}$}{ 
  	 \For{$i=1$ to $\ceil{2S/2^j}$}{
           \texttt{Augment$(G,M, 2^j)$};\\
	}	
  }
  \Return{$M$};
\end{algorithm}

We are now ready to proof our main theorem, which states that there is
a randomized $O(s^*\log s^*)$-time \CONGEST algorithm to compute a
maximum matching in an arbitrary undirected graph $G=(V,E)$.

\begin{proof}[\bf Proof of \Cref{thm:main}]
  We show that if all the nodes of a network graph $G$ are given an
  upper bound $S$ on the size $s^*$ of a maximum matching, a maximum
  matching can be computed in time $O(S\log S)$. The claim of the
  theorem then directly follows from \Cref{cor:matchingsize}.

  Starting with an initially empty matching $M$, the
  algorithm proceeds for $\ceil{\log(2S)}$ phases.  Let
  \texttt{Augment$(G,M,\ell)$} be the randomized protocol that is
  guaranteed by \Cref{lemma:pathalg}, i.e.,
  \texttt{Augment$(G,M,\ell)$} improves the matching $M$ iff there is
  an augmenting path of length at most $\ell$.  For
  $j= 1, \dots, \ceil{\log(2S)}$, in phase $j$, the algorithm calls
  \texttt{Augment$(G ,M, 2^j)$} at least $2S/2^j$ times (see
  \Cref{alg:maximum-matching}).

  We show by induction on $j$ that at the end of each phase $j$, the
  matching $M$ is of size $|M|>s^* - 2s^*/2^{j}$. To prove the
  induction base, we need to prove that after phase $1$, $|M|>s^*-2s^*/2^1=0$,
  which is clearly true (after phase $1$, $M$ is a maximal matching,
  which clearly is of size at least $1$). For the induction step,
  consider a phase $j\geq 2$. By the induction hypothesis, at the
  beginning of the phase, we have $|M|>s^*-2s^*/2^{j-1}$. In phase
  $j$, \texttt{Augment$(G,M,2^j)$} is called at least $2S/2^j\geq
  2s^*/2^j$ times. Hence, by \Cref{lemma:pathalg}, either the matching
  size is improved in each of these at least $2s^*/2^j$ calls to
  \texttt{Augment$(G,M,2^j)$} or there is no augmenting path of
  length at most $2^j$. In the first case, the matching $M$ at the end
  of the phase is of size at least $|M|>s^* -
  2s^*/2^{j-1}+2s^*/2^j=s^*-2s^*/2^j$. In the second case,
  \Cref{lem:aug-size} implies that $2s^*/(s^*-|M|)>2^j$ and thus we
  also have $|M|>s^* - 2s^*/2^j$. This concludes the induction on the
  phases. After phase $\ceil{\log(2S)}$, we have $|M| > s^* - 2s^*/2S
  \geq s^*-1$ and thus $|M|=s^*$.

  The bound on the running time follows because by
  \Cref{lemma:pathalg}, one call to \texttt{Augment$(G,M,2^j)$} has
  time complexity $O(2^j)$ and therefore each of the
  $O(\log S)=O(\log s^*)$ phases has a time complexity of
  $O(S)=O(s^*)$.
\end{proof}


	

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

